AUGCO: Augmentation Consistency-guided Self-training for Source-free Domain Adaptive Semantic Segmentation

Most modern approaches for domain adaptive semantic segmentation rely on continued access to source data during adaptation, which may be infeasible due to computational or privacy constraints. We focus on source-free domain adaptation for semantic segmentation, wherein a source model must adapt itself to a new target domain given only unlabeled target data. We propose Augmentation Consistency-guided Self-training (AUGCO), a source-free adaptation algorithm that uses the model's pixel-level predictive consistency across diverse, automatically generated views of each target image along with model confidence to identify reliable pixel predictions, and selectively self-trains on those. AUGCO achieves state-of-the-art results for source-free adaptation on 3 standard benchmarks for semantic segmentation, all within a simple to implement and fast to converge method.

==> sections/__latexindent_temp.tex <==
% \vspace{-7pt}
\section{Limitations \& Conclusion}
\label{sec:conclusion}
% \vspace{-5pt}

Despite \method's versatility, its effectiveness is limited by the correlation between predictive consistency and correctness, which varies across categories. Modifying source training to improve this correlation may be promising future work. Further, \method requires an extra forward pass and confidence thresholding, which makes it slightly slower than \texttt{TENT}~\cite{wang2021tent}. Finally, while \method seeks to make source-free adaptation more robust, such unsupervised training still has the potential to fail silently. A deeper investigation into the the failure modes of such methods is required before deployment in sensitive applications. Despite these limitations, we believe that \method is a step towards developing an effective source-free adaptation algorithm that can be used in the real-world at practical computational cost.


\noindent\textbf{Acknowledgements.} We thank Prithvijit Chattopadhyay for feedback on the draft. This work was supported in part by funding from the DARPA LwLL project.
